Gottesman Types for Quantum Programs

The Heisenberg representation of quantum operators provides a powerful technique for reasoning about quantum circuits, albeit those restricted to the common (non-universal) Clifford set H, S and CNOT. The Gottesman-Knill theorem showed that we can use this representation to efficiently simulate Clifford circuits. We show that Gottesman's semantics for quantum programs can be treated as a type system, allowing us to efficiently characterize a common subset of quantum programs. We also show that it can be extended beyond the Clifford set to partially characterize a broad range of programs. We apply these types to reason about separable states and the superdense coding algorithm.

==> eptcsdata.tex <==
\providecommand{\firstpage}{279}
\providecommand{\publicationstatus}{B. Valiron, S. Mansfield, P. Arrighi and P. Panangaden\\ (Eds.): Quantum Physics and Logic 2020 (QPL'20)\\
EPTCS 340, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.340.14}{10.4204/EPTCS.340.14}}
\pdfoutput=1

